ORIGIN: Blind detection of faint emission line galaxies in MUSE datacubes

One of the major science cases of the MUSE integral field spectrograph is the detection of Lyman-alpha emitters at high redshifts. The on-going and planned deep fields observations will allow for one large sample of these sources. An efficient tool to perform blind detection of faint emitters in MUSE datacubes is a prerequisite of such an endeavor. Several line detection algorithms exist but their performance during the deepest MUSE exposures is hard to quantify, in particular with respect to their actual false detection rate, or purity. {The aim of this work is to design and validate} an algorithm that efficiently detects faint spatial-spectral emission signatures, while allowing for a stable false detection rate over the data cube and providing in the same time an automated and reliable estimation of the purity. Results on simulated data cubes providing ground truth show that the method reaches its aims in terms of purity and completeness. When applied to the deep 30-hour exposure MUSE datacube in the Hubble Ultra Deep Field, the algorithms allows for the confirmed detection of 133 intermediate redshifts galaxies and 248 Lyman Alpha Emitters, including 86 sources with no HST counterpart. The algorithm fulfills its aims in terms of detection power and reliability. It is consequently implemented as a Python package whose code and documentation are available on GitHub and readthedocs.

==> old.tex <==
%%%%%%%%%%%%%%%%%%%
\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Diagrams/mainbloc.pdf}}
\caption{default}
\label{default}
\end{center}
\end{figure}

White light image et variance.
\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=.51\linewidth]{Figures/0_WhiteLight.pdf}{\includegraphics[width=.49\linewidth]{Figures/0_VAR.pdf}}}
% \centerline{\includegraphics[width=\linewidth]{Figures/0_VAR.pdf}}
\caption{`White light' image of the std-weighted data (log scale) and variance.}
\label{fig1}
\end{center}
\end{figure}


\subsection{Preprocessing}
$\Rho$ ($\brho$ or $\rho$) will denotes the RAW data , $\Sigma^2  \slash \sigma^2$ the cube of variance and $\Omega \slash \omega$ a  boolean cube mapping the existing data. 

as a preprocessing... to reduce the influence of extended sources a DCT is applied, this allow split the cube $\bY$ into two cubes. $\wbX$ the residual of the analysis will be cleaned of the principal perturbation and will contain the wanted sources. The second, $\wbC$,  will give a reliable estimation of the major extended sources with high continuum. Both cubes are also perturbed by the artifact contained into $\bY$.
Using an DCT atom based dictionary $\bD$ each spectra will be processed:
\begin{align}
\wc_\rho &= \bD \bD^T \rho \\
\wx_\rho &=  \rho - \wc_\rho
\end{align}

The cubes are then whitened by the given variance, using $\oslash$ to denotes element-wise division: 
\begin{align}
\wbX&= \wbX_\rho \oslash \Sigma \\
\wbC &= \wbC_\rho \oslash \Sigma
\end{align}
and are shown in Fig. \ref{fig_cont}

This preprocessing will help for further step. 
The obtained cubes are still suffering from instrumental artefacts, and in addition concerning the residual cube suffering from uncleaned continuum.
The estimated continuum cube will be used as a localization map of the extended sources.
In order to highlight the continuum part of each spectra and to reduce the influence of the artifact contained in the original data, each spectra of the continuum cube is cleaned from its own variance. 
\begin{align}
c&=\frac{\wc} {\sigma(\wc)}
\end{align}

The residual cube will receive a special cleaning process described in next section. 

%-----%

\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=.49\linewidth]{Figures/1_ContDCT.pdf}\includegraphics[width=.49\linewidth]{Figures/1_FaintDCT.pdf}}
% \centerline{\includegraphics[width=\linewidth]{Figures/1_FaintDCT.pdf}}
\caption{Estimated std-weighted continuum (log scale) and std-weighted residuals.}
\label{fig_cont}
\end{center}
\end{figure}

\subsection{Automatic source Guided Area Segmentation}
Typical MUSE data cube are sized by hundreds of billion of spatio spectral samples.
In addition the field of view can be incomplete as well as the spatial geometry of the observed data can be rotated.
In the next section the cleaning algorithm will be presented, however test shown that to achieve good results the cleaning process must be applied on data of a reasonable size. 
Too small data cube will be too much cleaned while too big cube will lead to slow convergence.
It become crucial in such a case to be able to segment the data cube into smaller area while preserving the sources content such as not splitting a source between two areas.

The second step of origin consists in an automatic, sources guided segmentation of the spatial dimension of the data cube which is illustrated in Fig. \ref{fig_seg}.
The first step of the spatial segmentation is to split the spatial dimension of the data cube into equal square areas. 
Depending on the spatial geometry some areas can contain missing data. 
In the specific example illustrated on the top right of the Fig. \ref{fig_seg} only the central sub cube is full. 
The background image of this figure is the energy of $c$ the continuum part of the data.
\begin{align}
\xi(c)&=\frac{1}{N_\lambda} \sum_\lambda c_\lambda^2 \approx \mu_c^2 + 1 = 1 + \left( \frac{1}{N_\lambda} \sum_\lambda c_\lambda  \right)^2
\end{align}
The square empirical mean being a reliable indicator of the spatially extended sources which possess an important continuum.
It will be used as a test to estimate the sources location 
\begin{align}
T[c]&=\xi(c)-1 \approx \chi^2_1
\end{align}
Which follow a $\chi^2$ distribution with one degree of freedom. 

In order to forbid some areas to be too small, a first fusion is applied.
It is simple merging which associate to the same label areas with a surface inferior an empirical value. 
After this fusion the border of the areas are still straight and can split sources between areas. 

Introducing a Probability of false alarm (PFA) of $20\%$ to compute a threshold $\gamma$ applied on the test: $T[c]>\gamma$ will give an estimate of the source location. 
The source splitting is then avoided by merging the detected sources area to the most probable sub area, the one which possess the biggest surface of the ambiguous source.

The automatic segmentation method will insure a maximum separation between sources by following a classification spirit. 
In each area, the convex enveloppe of the included sources is performed while preserving borders of others areas (source intrusion).
Then each area  grow using dilation to reach the final areas illustrated on the bottom left and right of the Fig. \ref{fig_seg} respectively.

\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=.49\linewidth]{Figures/A_step0.pdf}\includegraphics[width=.49\linewidth]{Figures/B_step0.pdf}}
 \centerline{\includegraphics[width=.49\linewidth]{Figures/C_step0.pdf}\includegraphics[width=.49\linewidth]{Figures/D_step0.pdf}}
\caption{Example of a sources guided automatic segmentation.}
\label{fig_seg}
\end{center}
\end{figure}

\subsection{Greedy PCA}
The idea behind the greedy PCA is to clean the residual cube while preserving the emission line by an iterative process involving a PCA. 
To do so, the processing will remove the influence of the instrumental artefacts and of the uncleaned continuum sources with a the condition to not remove everything.  
Considering a Normal distribution of the noise, a test based on a second order moment will emphasize spectra with abnormal variance and mean.
Under this assumption this will help to separate nuisances spectra which suffer from perturbations and background spectra. 
The test will be explained after and will also drives the stopping criteria.
Nuisances spectra contains the continuum part of the sources and of the instrumental artefacts.
Background spectra will essentially contains noise and the source of interest. 
The emission line being a convolved impulse in noise will not affect the mean and or the variance of a spectra, parameters measured by the test.
In order to keep the homogeneity of the result, the nuisances part will be orthogonalized with the signature of the background part.
This step will insure that a cleaned area of nuisances will at least fit the statistical properties of the background.
Then, a signature of the perturbations will be removed from the whole data cube. 
Applying the cleaning on the full data will remove long term influence of the perturbation on background spectra for which the perturbation is low but still existing.

For a spectra, under normal distribution assumption of the noise, the second order moment test is given by:
\begin{align}
T[x]&=\frac{1}{N_\lambda} \sum_\lambda x_\lambda^2 \approx \mu_x^2 + \sigma_x^2
\end{align}
Where $ \mu_x$ and $\sigma_x$ are the empirical means and variance of $x$.

A PFA based threshold $\gamma$ is computed on the statistics of the input residual $\wX$ and is used to perform the separation nuisances/background, the threshold is then not updated.  
The iterative process stop when all the spectra are considered as being part of background or a pre defined maximum iteration number. 

\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Figures/2_PCA_tresh_All.pdf}} 
 \centerline {\includegraphics[width=\linewidth]{Figures/2_FullInitPCA.pdf}}
  \centerline{\includegraphics[width=\linewidth]{Figures/2_IterationPCA.pdf}}
 \centerline{\includegraphics[width=\linewidth]{Figures/2_PCA.pdf}}
\caption{Top : The nine tests (left) and the zones classified as nuisances (black) (right). Bottom : Number of iterations of greedy PCA for each spectrum (left)
and  PCA residuals (right).}
\label{fig3}
\end{center}
\end{figure}

Considering the perturbed matrix of the residual $\wX$ The principal step are the following: 
\begin{itemize}
\item the residual matrix $\wX$ is split into nuisance and background part denoted $\wX^n$ and $\wX^b$ respectively 
\item a signature's vector $x_b$ of size $N_\lambda$ is computed by averaging $\wX^b$ among the spatial dimension
\item The perturbed matrix to clean is then formed by orthogonalization: $S = (x_b^T x_b)^{-1} {x_b}^T \wX^n$
\item The principal eigenvector $\vs$ of $S$ is computed via a sparse PCA 
\item the residual matrix is cleaned: $\wX = (\vs^T \vs)^{-1} {\vs}^T \wX$
\end{itemize}





\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Figures/2_WhitePCA.pdf}}
\caption{and white light image of std-weighted PCA residuals.}
\label{fig4}
\end{center}
\end{figure}

\subsection{Weighted correlations and local maxima}

We assume in this step that the method described in the previous section cleaned the data from extended sources. 
The residual data is composed by noise and convolved line. 
The convolution is spatio-spectral.
As an approximation the lines are modeled by gaussian profiles although they can be not symmetric

\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Figures/0_Profiles.pdf}}
\caption{Profiles and spatial projection of the PSF.}
\label{fig_profiles}
\end{center}
\end{figure}

blah blah about the TGLR, normalisation, convolution and spectral gain
The result of the test will give a reliable estimation of the sources location and his the core of the detection process of ORIGIN.
The maxmap: the maximum other the channel of the maximum correlation over the profiles is shown on the top of Fig. \ref{maxmaps}.
When a sample gives a high correlation with a profile, its  close spatio-spectral environment gives, in general, also and the detected sources are not punctual.
Addition treatments are needed, the test could be brutally thresholded but the question of finding the real position of a source inside an extended, and in general non convex, 3D area would need to be solved.

To disambiguate the probable sources contained in the same envelope of profiles local maximum are computed.
The resulting sparse cube is illustrated over is maximum component in Fig. \ref{maxlocmaps}

For calibration purpose we extract two informative cubes from the correlations test. 
The first one is the cube over the profiles which maximize the correlations.
The second, the one which minimize the correlation and is exactly the same as maximizing the correlation on the opposite of the data.  




\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Figures/3_MAXMAP.pdf}}
  \centerline{\includegraphics[width=\linewidth]{Figures/3_MAXMAP_min.pdf}}
\caption{Map of the maxima of the weighted correlation on the data (top) and the opposite of the data (bottom)}
\label{maxmaps}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Figures/4_MAXlocalMAP.pdf}}
  \centerline{\includegraphics[width=\linewidth]{Figures/4_MAXlocalMAP_min.pdf}}
\caption{Map of the local maxima of the weighted correlation on the data (top) and the opposite of the data (bottom) (maximum for each spectrum)}
\label{maxlocmaps}
\end{center}
\end{figure}


\subsection{Fidelity estimation and thresholding}

\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Figures/5_Segmentation_theshold.pdf}}
  \centerline{\includegraphics[width=\linewidth]{Figures/5_Background_purity.pdf}}
    \centerline{\includegraphics[width=\linewidth]{Figures/5_Sources_purity.pdf}}
\caption{Segmentation, estimated fidelity for bright and background zones}
\label{fig7}
\end{center}
\end{figure}


\subsection{Line estimation}
\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Figures/0_25_estimate_Mean_STD_BIAS_theoemp.pdf}}
  \centerline{\includegraphics[width=\linewidth]{Figures/2_abs_25_SCORE.pdf}}
%    \centerline{\includegraphics[width=\linewidth]{Figures/5_Sources_purity.pdf}}
\caption{Estim}
\label{fig8}
\end{center}
\end{figure}

%%%%%%%%%%%
\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Diagrams/preproc.pdf}}
\caption{default}
\label{default}
\end{center}
\end{figure}

\subsection{Greedy PCA}
\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Diagrams/pcaseuil.pdf}}
\caption{default}
\label{default}
\end{center}
\end{figure}

\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Diagrams/greedypca.pdf}}
\caption{default}
\label{default}
\end{center}
\end{figure}

\subsection{Weighted correlations}
\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Diagrams/correl.pdf}}
\caption{default}
\label{default}
\end{center}
\end{figure}

\subsection{Segmentation}
\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Diagrams/segmentation.pdf}}
\caption{default}
\label{default}
\end{center}
\end{figure}


\subsection{Fidelity estimation}
\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Diagrams/thresh.pdf}}
\caption{default}
\label{default}
\end{center}
\end{figure}

\subsection{Line estimation}
\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Diagrams/gridding.pdf}}
\caption{default}
\label{default}
\end{center}
\end{figure}

\subsection{Merging}
\begin{figure}[htbp]
\begin{center}
 \centerline{\includegraphics[width=\linewidth]{Diagrams/merging.pdf}}
\caption{default}
\label{default}
\end{center}
\end{figure}
